Graph space: using both geometric and probabilistic structure to evaluate statistical graph models

Statistical graph models aim at modeling graphs as random realization among a set of possible graphs. One issue is to evaluate whether or not a graph is likely to have been generated by one particular model. In this paper we introduce the edit distance expected value (EDEV) and compare it with other methods such as entropy and distance to the barycenter. We show that contrary to them, EDEV is able to distinguish between graphs that have a typical structure with respect to a model, and those that do not. Finally we introduce a statistical hypothesis testing methodology based on this distance to evaluate the relevance of a candidate model with respect to an observed graph.

==> sec_mod_comparison.tex <==
Now let's have a look at a different, yet related, problem. Suppose we have two models associated with different graph spaces and we wonder if it is possible to use one in place of the other. The EDEV measure can be used to check how similar those graph spaces are. For example, if we consider the configuration model. For a degree sequence $K = (k_i^{in}, k_i^{out})_{i \in V}$, the associated microcanonical ensemble is:
\[
\Omega_K = \{G = (V,E) \mid \forall i \in V, \mathrm{deg^{in}}(i) = k_i^{in}, \mathrm{deg^{out}}(i) = k_i^{out}\}
\]
It is known to be very difficult to compute the cardinal of this ensemble \cite{bender_asymptotic_1978}, and thus the probability $\mathbb{P}[W(i,j) = w] = \frac{|\{H \in \Omega_K \mid W_H(i,j) = w\}|}{|\Omega_K|}$ that a given edge $(i,j)$ has weight $w$. To ease this computation, a relaxation has been proposed in \cite{giona_casiraghi_generalised_2018}, called the soft configuration model, that considers a larger set of graphs
\[
\Omega_K' = \{G = (V,E) \mid |E| = m\}
\]
with an associated probability distribution such that the degree sequence $K$ is followed in average:
\[
\mathbb{P}[G] = \frac{\prod_{i,j \in V}\binom{\Xi_{ij}}{W_G(i,j)}}{\binom{M}{m_G}}
\]
with $\Xi_{ij} = k_i^{out} k_j^{in}$ and $M = \sum_{i,j \in V} \Xi_{ij}$.

The main advantage of this relaxation is that all probabilities become much easier to compute. The problem is that beyond the fact that the degree sequence is followed on average, we have little control on which graphs have been added to the model ensemble and the impact it has on the model properties. In fact, authors of \cite{giona_casiraghi_generalised_2018} cannot provide an evaluation of the quality of their approximation. To check for that, we compare the configuration model and the soft configuration model for different degree sequence on $n = 100$ nodes:
\begin{enumerate}
\item Constant degree distribution, with degree $k$ ranging from 2 to 100.
\item Arithmetic degree distribution, with $k_i = k * i$, and $k = 1, 2, 3, 4, 5$
\item Star degree distribution, with $k_0 = k$ and $\forall i \geq 1, k_i = 1$, k ranging from 1 to 1000.
\end{enumerate}
For each degree sequence, a graph is generated according to the stub-shuffling algorithm described in \cite{newman2001random}. Then, its edit distance expected value is computed analiticaly for the soft configuration model, and for the configuration model we compute it by averaging its edit distance over 50 other graphs with the same degree sequence. Results are shown on figure \ref{cfm_vs_scfm} with error bars for the configuration model curve.

\begin{figure}[h]
  \includegraphics[height=0.3\textheight]{Images/constant_degree_dist_cfm.png}
  \includegraphics[height=0.3\textheight]{Images/arith_degree_dist_cfm.png}
  \includegraphics[height=0.3\textheight]{Images/star_degree_dist_cfm.png}  
  \caption{\textbf{Configuration model vs soft configuration model.} First curve is for the constant degree distribution, second one is for arithmetic degree distribution and the third is for the star degree distribution.\label{cfm_vs_scfm}}
\end{figure}

We observe that for the constant and arithmetic distribution, both models give remarkably similar results. This means that, on average, the soft configuration model generates graphs which share about the same number of edges with graphs generated using the configuration model as the configuration model itself. This is useful in practice, because it means that the weight probability distribution derived analytically from the soft configuration model is close to the configuration model one, which can only be approximated using sampling. On the other hand, we observe that in the case of a star degree distribution, results diverge. This can be explained by the fact that in this situation, the soft configuration model tends to produce a lot more self-loop on the central node than the configuration model would. 

These observations show how studying graph space may reveal similarities or discrepancies between models and in this case help determine the validity range of the soft configuration model approximation.

==> statistical_hypothesis_testing.tex <==
This methodology can be formalized using statistical hypothesis testing. Let's say we have a graph $G$ and a model $M$ (possibly obtained by fitting some parameters on $G$). We want to test the hypothesis $\mathcal{H}$: ``the observed graph $G$ has been generated by the candidate model $M$". 

We do so in the following way:
\begin{enumerate}
    \item Choose a confidence level $\delta$, for example $0.01$.
    \item Generate a random sample from the candidate model $\mathcal{S} \subset \Omega_M$, of $n_b$ test graphs.
    \item Infer the probability distribution $\mathbb{P}_{ed}$ of $\mathrm{EDEV}(H, \Omega_M)$ for $H \in \Omega_M$ from the sample $\mathcal{S}$. 
    \item Compute the probability \[p = \mathbb{P}_{ed}[|\mathrm{EDEV}(H, \Omega_M) - d_M| \geq |\mathrm{EDEV}(G, \Omega_M) - d_M|]\]
    \item If $p < \delta$, it means that the probability that $G$ was generated by $M$ is inferior to $\delta$ and the hypothesis $\mathcal{H}$ can be rejected. 
\end{enumerate}

{\color{red}
The most efficient and rigorous method to infer the probability distribution $\mathbb{P}_{ed}$ would be to characterize precisely the distribution $\mathbb{P}_{ed}$ for various models and to derive the parameters of the distribution directly from the parametrization of the model. However, this would imply to further investigate the structure of the microcanonical ensemble.} As a first approximation, given the concentration of the samples around the mean, we assume that this distribution is normal, so we only need to infer the mean $d_M$ and the standard deviation $\sigma_M$ of the distribution. This assumption is verified on the models described in the previous subsection by comparing the cumulative distribution function of the sample with the one of the corresponding normal distribution. An example is shown in figure \ref{sample_vs_normal_cdf}. The Shapiro-Wilk test returned a p-value below $0.05$ (around $0.01$) for $2$ of the $10$ models. This means that the normal distribution can only be considered a rough estimate in general, but it can be considered good enough as a first approximation. 

{\color{red} We then infer the parameters of this normal distribution based on a sample $\mathcal{S}$ of graphs in the microcanonical ensemble. This technique would not be adapted to the study of large-scale real networks as it requires to uniformly sample the microcanonical ensemble. For instance, in the case of the simple graph formulation of the configuration model, the main solution to generate uniform samples inside the microcanonical ensemble is to use the edge-switching algorithm described in \cite{fosdick2018configuring}, which requires high mixing time to ensure a uniform distribution of the outcomes. In our case, to avoid those issues we focused on relatively small graphs for which uniform random sampling is not prohibitive.
}

\begin{figure}[htb]
    \centering
    \includegraphics[width=0.7\textwidth]{normal_check.png}
    \caption{Comparison between the empirical distribution of the edit distance expected value for graphs generated with a configuration model ($CFMD_0$) and the normal distribution with the same mean and standard deviation.}
    \label{sample_vs_normal_cdf}
\end{figure}
    
\begin{figure}[htb]
    \begin{center}
    \includegraphics[scale=0.5]{Images/spatial_graph.png}
    \end{center}
    %\caption[Spatial graph generated using the waxman random geometric model.]
    \caption{\label{spatial_graph} Spatial graph generated using the Waxman random geometric model. $100$ nodes are randomly distributed in a $[0,1]\times[0,1]$ square. They are then connected with a probability depending on the distance $d$ between nodes: $p(d) = 10\exp\left(\frac{d}{0.05L}\right)$, with $L$ the maximum distance between two nodes. Communities are computed using graph-tool
    %\footnotemark.} %
    (\url{https://graph-tool.skewed.de/}).}
\end{figure}
%\footnotetext{\url{https://graph-tool.skewed.de/}}

Let's consider a situation in which one wishes to evaluate the relevance of the block structure computed on a graph $G$, with a weight matrix $W_G$. Whatever the graph, and the partition $B = (b_1, \dots, b_p)$ of its $n$ nodes, it is always possible to define $M \in \mathcal{M}_p(\mathbb{N})$ as
\[ \forall i,j \in \llbracket 1, p \rrbracket, M[i,j] = \sum_{u \in b_i, v \in b_j} W_G[u,v]\]
such that $G \in \Omega_{SBM(n, B, M)}$. The objective is to evaluate whether this stochastic blockmodel is a relevant model of $G$. An even trickier question is to evaluate whether any stochastic blockmodel can be a relevant model. In particular, spatial models can generate graphs with groups of nodes densely connected due to their
position rather than to block membership. An example of such a graph is shown in figure \ref{spatial_graph}. It may then be hard to tell whether the blocks found are indeed a legitimate model of the observed graph or should be considered as artefacts, consequences of the underlying spatial structure.

%\begin{figure}[H]
%    \begin{center}


To illustrate how statistical hypothesis testing allows to address this issue, we consider eight models: four stochastic blockmodels and four Waxman models for random geometric graphs\footnote{\url{https://networkx.org/documentation/stable/reference/generated/networkx.generators.geometric.waxman\_graph.html}} with different sets of parameters. The Waxman model for spatial graphs allows to easily control the strength of the spatial structure, by tuning the speed at which edge probability decays as the distance between nodes rises. The number of nodes is fixed to $n = 100$ and the parameters are fixed such as to ensure a density $d$ around $0.036$. All stochastic blockmodels use a node partition in four blocks of $25$ nodes, with a block adjacency matrix of the form:
\[
\begin{bmatrix}
    m_{int} & m_{ext} & m_{ext} & m_{ext} \\
    m_{ext} & m_{int} & m_{ext} & m_{ext} \\
    m_{ext} & m_{ext} & m_{int} & m_{ext} \\
    m_{ext} & m_{ext} & m_{ext} & m_{int}
\end{bmatrix}
\]  
The four stochastic blockmodels are then defined by:
\begin{enumerate}
    \item $M_0$: $m_{int} = 90$, $m_{ext} = 0$    
    \item $M_1$: $m_{int} = 75$, $m_{ext} = 5$
    \item $M_2$: $m_{int} = 60$, $m_{ext} = 10$
    \item $M_3$: $m_{int} = 45$, $m_{ext} = 15$
\end{enumerate}
This way, the graphs generated using $SBM_0$ are made of perfectly separated blocks of nodes, while those generated by $SBM_3$ have blocks with as many internal and external edges.

For the Waxman models, we also consider four parameter sets:
\begin{enumerate}
    \item $M_4$: $\alpha = 0.1$, $\beta = 1$
    \item $M_5$: $\alpha = 0.08$, $\beta = 1.6$
    \item $M_6$: $\alpha = 0.06$, $\beta = 2.7$
    \item $M_7$: $\alpha = 0.04$, $\beta = 8.5$
\end{enumerate}
The lower the value of $\alpha$, the stronger the spatial structure.

With each model $M_i$, we generate $8$ graphs $(G_{i,j})_{j \in \llbracket 0, 7 \rrbracket}$. On each of those observed graph, we find the minimum entropy node partition $B_{i,j}$ using graph tools, and fit a candidate stochastic blockmodel $SBM_{i,j}$ on $G_{i,j}$ based on this node partition. We then evaluate the relevance of this stochastic blockmodel using the previously described methodology. We use a confidence level $\delta$ of $0.01$ and a sample size $n_b = 200$. The probabilities $p_{i,j}$ obtained are plotted in figure \ref{p_value}.

\begin{figure}
    \centering
    \includegraphics[scale=0.35]{Images/p_value_spa_sbm.png}
    \caption{For each model $M_i$ in ordinate, and each graph number $i$ in abscissa, we compute the probability $p_{i,j}$ that a graph generated using $SBM_{i,j}$ has a normalized edit distance expected value to $SBM_{i,j}$ further away from the mean value $d_{i,j}$ than $G_{i,j}$. The probability is plotted in heatmap.}
    \label{p_value}
\end{figure}

We observe that for all graphs generated by stochastic block models but one, $p_{i,j} > 10^{-2} = \delta$. On the other hand, for all spatial graphs $p_{i,j} < \delta$. This means that the hypothesis "$G_{i,j}$ has been generated by the candidate stochastic block model $SBM_{i,j}$" is rejected for all $32$ spatial graphs, and for the $8^{th}$ graph generated by $SBM_2$. Let's stress again that a probability $p_{i,j}$ superior to $\delta$ does not mean that $SBM_{i,j}$ is the right model for $G_{i,j}$. It only means that there is not enough statistical evidence to reject it.

These results show that, on $32$ spatial graphs generated with various sets of parameters, the statistical hypothesis testing methodology is able to correctly identify that the block structure found is not a relevant model, despite being the solution maximizing the likelihood. This result is not trivial. {\color{red} Indeed, the fact that this partition is the most likely according to the entropy definition of likelihood means that the block identified are characterized by a specific connection density which cannot be explained by random fluctuations. However, as the likelihood is maximized on a set of models which does not contain the Waxman model used to generate the graph, this estimator is not able to recognize that its structure would be even better explained using a spatial model}. What is more, this methodology manages to reject the block structure for all spatial graphs while spuriously rejecting it for only one out of $32$ graphs originally generated with a stochastic blockmodel. In other words, {\color{red}there is no false positive, and only one false negative.}

Strictly speaking, these results only allow to rule out one node partition. As the block structure tested were fitted on the observed graphs using minimum entropy, one could argue that ruling out this partition implies that no other node partition can lead to a relevant model. Yet, for most real graphs, there is more than one plausible node partition and minimizing the entropy of a partition is a stochastic process. Therefore, the experiment should be performed more than once to conclude that the observed graph has no block structure.
